Linting Style and Substance in READMEs

READMEs shape first impressions of software projects, yet what constitutes a good README varies across audiences and contexts. Research software needs reproducibility details, while open-source libraries might prioritize quick-start guides. Through a design probe, LintMe, we explore how linting can be used to improve READMEs given these diverse contexts, aiding style and content issues while preserving authorial agency. Users create context-specific checks using a lightweight DSL that uses a novel combination of programmatic operations (e.g., for broken links) with LLM-based content evaluation (e.g., for detecting jargon), yielding checks that would be challenging for prior linters. Through a user study (N=11), comparison with naive LLM usage, and an extensibility case study, we find that our design is approachable, flexible, and well matched with the needs of this domain. This work opens the door for linting more complex documentation and other culturally mediated text-based documents.

==> figures/comaprision-table-revisit.tex <==

% --- colors ---
\definecolor{lred}{HTML}{E57373}
\definecolor{lgreen}{HTML}{81C784}
\definecolor{lorange}{HTML}{FFB74D}

% --- tiny label boxes ---
\newcommand{\lBox}[2]{\colorbox{#1!35}{\strut\textsf{#2}}}
\newcommand{\lBoxSmall}[2]{\colorbox{#1!35}{\strut\scriptsize\textsf{#2}}}

% --- yes/maybe/no macros ---
\newcommand{\no}{\lBoxSmall{lred}{N}}
\newcommand{\maybe}{\lBoxSmall{lorange}{P}}
\newcommand{\yes}{\lBoxSmall{lgreen}{Y}}

\begin{figure*}[t]

    \small
    \centering
    \footnotesize
    \setlength{\tabcolsep}{0.1pt}
    \setlength{\fboxsep}{4pt} 
    {
        \begin{tabular}{rcccccccccccccccccccccccccccc}
      % \toprule  
Name\hspace{0.075in} & 
\rot{\lint{execution}} & 
\rot{\lint{code-formatting}} & 
\rot{\lint{link-formatting}} & 
\rot{\lint{link-validation}} & 
\rot{\lint{formatting-and-styling}} & 
\rot{\lint{style-consistency}} & 
\rot{\lint{structure}} & 
\rot{\lint{terminology}} & 
\rot{\lint{sensitive-content}} & 
\rot{\lint{sections completeness}} & 
\rot{\lint{repetition}} & 
\rot{\lint{sentence-length}} &  
\rot{\lint{TOC}} & 
\rot{\lint{navigation}} &  
\rot{\lint{no-jargon}} & 
\rot{\lint{visual-clarity}} & 
\rot{\lint{alt-text}} & 
\rot{\lint{cross-platform}} & 
\rot{\lint{availability}} & 
\rot{\lint{objectivity}} & 
\rot{\lint{hate-words}} & 
\rot{\lint{spelling-and-grammar}} & 
\rot{\lint{content-variety}} & 
\rot{\lint{date-related}} &  
\rot{\lint{end-with-new-line}} & 
\rot{\lint{emoji-Lint}}\\
\midrule  
% \ti{Don't know we need it or not}

& \multicolumn{4}{c}{\roundTag{1.4cm}{lpurple}{Accuracy}}
& \multicolumn{4}{c}{\roundTag{1.4cm}{lpurple}{Consistency}}
% Security
& \multicolumn{1}{c}{\roundTag{0.35cm}{lpurple}{S}}
& \multicolumn{3}{c}{\roundTag{1.05cm}{lpurple}{Concise}}
& \multicolumn{6}{c}{\roundTag{2.3cm}{lpurple}{Accessibility}}
% Availability
& \multicolumn{1}{c}{\roundTag{0.35cm}{lpurple}{V}}
% Objectivity
& \multicolumn{1}{c}{\roundTag{0.35cm}{lpurple}{O}}
% Reputation
& \multicolumn{1}{c}{\roundTag{0.35cm}{lpurple}{R}}
% Quality
& \multicolumn{1}{c}{\roundTag{0.35cm}{lpurple}{Q}}
% Appearance
& \multicolumn{1}{c}{\roundTag{0.35cm}{lpurple}{A}}
& \multicolumn{3}{c}{\roundTag{1.05cm}{lpurple}{Others}} \\

% \cmidrule(lr){2-5}
% \cmidrule(lr){6-9}
% \cmidrule(lr){10-10}
% \cmidrule(lr){11-13}
% \cmidrule(lr){14-19}
% \cmidrule(lr){20-20}
% \cmidrule(lr){21-21}
% \cmidrule(lr){22-22}
% \cmidrule(lr){23-23}
% \cmidrule(lr){24-24}
% \cmidrule(lr){25-27}


\midrule  
% Name \hspace{1mm} & 
% \multicolumn{4}{c|}{Acc./Reliability} & 
% \multicolumn{4}{c|}{Consistency} & 
% Security & 
% \multicolumn{1}{c|}{Timeliness }& 
% \multicolumn{3}{c|}{Concise}& 
% \multicolumn{6}{c|}{Accessibility}& 
% \multicolumn{1}{c|}{Availability}& 
% \multicolumn{1}{c|}{Objectivity}& 
% % \multicolumn{0}{c|}{Efficiency}& 
% \multicolumn{1}{c|}{Reputation}& 
% \multicolumn{2}{c|}{Value-added}& 
% \multicolumn{1}{c|}{Appeal}& 
% \multicolumn{3}{c|}{Others}
% \\
% \midrule  
markdownlint~\cite{markdownlint_ruby} \hspace{1mm} &  \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no \\ 
DavidAnson markdownlint~\cite{markdownlint_node} \hspace{1mm} &  \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \maybe & \no & \no & \yes & \no \\
mdformat~\cite{mdformat} \hspace{1mm} &  \no & \yes & \yes & \no & \maybe & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\ 
remark-lint~\cite{remarklint} \hspace{1mm} &  \no & \yes & \yes & \yes & \yes & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \yes & \yes \\
textlint~\cite{textlint} \hspace{1mm} &  \no & \no & \yes & \yes & \yes & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \yes & \no & \maybe & \no & \no \\ 
proselint~\cite{proselint} \hspace{1mm} &  \no & \no & \yes & \yes & \no & \maybe & \no & \maybe & \yes & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \yes & \yes & \yes & \no & \maybe & \no & \no \\ 
vale~\cite{vale} \hspace{1mm} &  \no & \yes & \no & \no & \no & \maybe & \no & \maybe & \no & \no & \maybe & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no \\ 
content-linter~\cite{github_content_linter} \hspace{1mm} &  \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \maybe & \no & \maybe & \yes & \no \\ 
alex~\cite{alex} \hspace{1mm} &  \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no \\ 
% webhint~\cite{webhintio_org} \hspace{1mm} &  \no & \no & \yes & \yes & \maybe & \maybe & \no & \no & \yes & \no & \no & \yes & \no & \maybe & \no & \yes & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no \\
write-good~\cite{writegood} \hspace{1mm} &  \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \maybe & \no & \no & \no & \no \\ 
standard-readme~\cite{standardreadme} \hspace{1mm} &  \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\ 
awesome-lint~\cite{awesome_lint} \hspace{1mm} &  \no & \yes & \yes & \yes & \yes & \yes & \maybe & \maybe & \no & \maybe & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \yes & \no \\
grammarly~\cite{grammarly_website} \hspace{1mm} &  \no & \no & \maybe & \no & \no & \no & \no & \maybe & \no & \no & \maybe & \yes & \no & \no & \yes & \no & \no & \no & \no & \no & \yes & \yes & \no & \yes & \no & \no \\ 
\hline
\textbf{\emph{\system{}}} \hspace{1mm} &  \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes \\
 \bottomrule
        \end{tabular}}\\[1em]
        
            \textbf{Y} = Supported, \textbf{N} = Not Supported, \textbf{P} = Partially Supported. If a tool supports custom rules (such as via plugins), if implementation is straight it is marked \textbf{Y} and \textbf{P} otherwise. \\
            \roundTag{0.35cm}{lpurple}{S} = Security,
            \roundTag{0.35cm}{lpurple}{V} = Availability,
            \roundTag{0.35cm}{lpurple}{O} = Objectivity,
            \roundTag{0.35cm}{lpurple}{R} = Reputation,
            \roundTag{0.35cm}{lpurple}{Q} = Quality,
            \roundTag{0.35cm}{lpurple}{A} = Appearance
    \caption{
    % \am{gross}\system{} is not the first documentation linter, but its approach is the most general.
    Prior tools have explored different approaches to linting markdown files in general and in \readmes{} specifically. 
    However, most tools have focused on either markdown style (\eg{} correct markdown usage) or on natural language style (\eg{} avoiding hateful terms). 
    Here we draw a sample of representative lints from across \citeetals{tang2023evaluating} documentation typology (denoted in  \roundTag{0.35cm}{lpurple}{purple}) for a variety of linters. While there are other linters and other lints, this collection offers a representative sample of the type of functionality available. 
    Lastly, this list centers only markdown evaluation, although some of the tools considered here, such as Vale~\cite{vale} include support for a range of other documentation formats (such as reStructuredText). 
    Additional details about this coding are available in the supplementary materials.
    % For instance \lint{Execution} checks if the code in a particular code snippet can be executed, while \am{another example}.  
    % Here we show whether a collection of such tool
    % Here we show all of the markdown and documentation linters with their supported lint rules.
    % These rules range widely across \am{those people's} categories. 
    % \am{add blocks to sections, highlight somewhere what we clipped}
    % \ki{Where did the columns come from? Are they from Tang and Nadi and Treude et al.? Are they all of them? Is there supplemental where I can see how each criteria was interpreted? If the design space is the contribution, where is it described?}
    }
    \Description{
A comparison table shows different linting tools and the quality checks  they support compared to LintMe tool. In total there are 13 rows for 13 different linting tool: markdownlint, mdformat, remark-lint, textlint, proselint, vale, content-linter, alex, write-good, standard-readme, awesome-lint, and grammarly. 
% 
The upper part of the table shows rules listed as vertical labels along columns, with subgroup headings placed below them. This include, accuracy and reliability, consisting of rules such as execution, code formatting, link formatting, and link validation. Consistency consists of rules such as formatting/styling, structure, and terminology. Security consists of rules such as sensitive content and best practices. 
Timeliness stands alone without group. 
Conciseness consists of rules such as section completeness, repetition, sentence length, and too concise.
Accessibility consists of rules such as navigation, no-jargon, visual clarity, alt text, and cross platform. 
Availability and objectivity also stand alone without groups. 
Reputation consists of rules on hate words. 
Quality checks consists of rules such as spelling and grammar rules. 
Appearance consists of rule on content variety. 
Other rules includes date related, end with new line, emoji lint, and translations.
% 
In the table, if a linting tool can flag rule, it is marked as Y; partial support is marked as P; and not supported marked as N. Colors reinforce this: Y with green, P with yellow, and N with red. From this table, if the linting tools is able to flag one of the rules, it will have Y, partially support P and not supported as N. With colors also telling the same thing with Y green, P yellow, N red. Most tools cover only handful of rules, by contrast, LintMe is the only tool that supports every rule with Y across the columns.
    }
        \label{tab:design-space}
        \vspace{-2em}
\end{figure*}

% \begin{table*}[t]
%     \caption{Design space of markdown and documentation linters with their supported lint rules \am{move legend down and add blocks to sections, highlight somewhere what we clipped}}
%     \label{tab:design-space}
%     \small
%     \centering
%     \setlength{\tabcolsep}{0.9pt}
%     \setlength{\fboxsep}{4pt} 
%     {
%         \begin{tabular}{lcccccccccccccccccccccccccc}
%       \toprule  
% Name & \rot{Execution} & \rot{Code formatting} & \rot{Link formatting} & \rot{Link validation} & \rot{Formatting and Styling} & \rot{Style consistency} & \rot{Structure} & \rot{Terminology} & \rot{Sensitive content} & \rot{Sections Completeness} & \rot{Repetition} & \rot{Sentence Length} &  \rot{TOC} & \rot{Navigation} &  \rot{No jargon} & \rot{Visual Clarity} & \rot{Alt Text} & \rot{Cross Platform} & \rot{Availability} & \rot{Objectivity} & \rot{Hate words} & \rot{Spelling and Grammar} & \rot{Content Variety} & \rot{Date related} &  \rot{End with new line} & \rot{Emoji Lint}\\
% \midrule  
% markdownlint~\cite{markdownlint_ruby} \hspace{1mm} &  \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no \\ 
% DavidAnson markdownlint~\cite{markdownlint_node} \hspace{1mm} &  \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \maybe & \no & \no & \yes & \no \\
% mdformat~\cite{mdformat} \hspace{1mm} &  \no & \yes & \yes & \no & \maybe & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\ 
% remark-lint~\cite{remarklint} \hspace{1mm} &  \no & \yes & \yes & \yes & \yes & \yes & \maybe & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \yes & \yes \\
% textlint~\cite{textlint} \hspace{1mm} &  \no & \no & \yes & \yes & \yes & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \yes & \no & \maybe & \no & \no \\ 
% proselint~\cite{proselint} \hspace{1mm} &  \no & \no & \yes & \yes & \no & \maybe & \no & \maybe & \yes & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \yes & \yes & \yes & \no & \maybe & \no & \no \\ 
% vale~\cite{vale} \hspace{1mm} &  \no & \yes & \no & \no & \no & \maybe & \no & \maybe & \no & \no & \maybe & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no \\ 
% content-linter~\cite{github_content_linter} \hspace{1mm} &  \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \maybe & \no & \maybe & \yes & \no \\ 
% alex~\cite{alex} \hspace{1mm} &  \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no \\ 
% webhint~\cite{webhintio_org} \hspace{1mm} &  \no & \no & \yes & \yes & \maybe & \maybe & \no & \no & \yes & \no & \no & \yes & \no & \maybe & \no & \yes & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no \\
% write-good~\cite{writegood} \hspace{1mm} &  \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \maybe & \no & \no & \no & \no \\ 
% standard-readme-preset~\cite{standardreadme} \hspace{1mm} &  \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no \\ 
% awesome-lint~\cite{awesome_lint} \hspace{1mm} &  \no & \yes & \yes & \yes & \yes & \yes & \maybe & \maybe & \no & \maybe & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \yes & \no \\
% grammarly~\cite{grammarly_website} \hspace{1mm} &  \no & \no & \maybe & \no & \no & \no & \no & \maybe & \no & \no & \maybe & \yes & \no & \no & \yes & \no & \no & \no & \no & \no & \yes & \yes & \no & \yes & \no & \no \\ 
% \hline
% \textbf{\emph{LintMe}} &  \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes \\
%  \bottomrule
%         \end{tabular}}\\
%             \textbf{Y} = Supported, \textbf{N} = Not Supported, \textbf{P} = Partially Supported.

% \end{table*}

% \begin{table*}[t]
%     \caption{Design space of markdown and documentation linters with their supported lint rules \am{move legend down and add blocks to sections, highlight somewhere what we clipped}}
    

%     \label{tab:design-space}
%     \footnotesize
%     \centering
%     \setlength{\tabcolsep}{0.9pt}
%     \setlength{\fboxsep}{2pt} 
%     {
%         \begin{tabular}{r
%         |cccc|
%         cccc|
%        cccc| cc|
%        cc|ccc|ccccccc|c|cc|ccccccccccccccccccccccccccccccccccccccccccccccccccccc}
%       % \toprule  
% % Name & \rot{Checkable} & \rot{Customizable} & \rot{Blamable} & \rot{Fixable} & \rot{Execution} & \rot{Code formatting} & \rot{Link formatting} & \rot{Link validation} & \rot{Formatting and Styling} & \rot{Style consistency} & \rot{Structure} & \rot{Terminology} & \rot{Sensitive content} & \rot{Sections Completeness} & \rot{Repetition} & \rot{Sentence Length} &  \rot{TOC} & \rot{Navigation} &  \rot{No jargon} & \rot{Visual Clarity} & \rot{Alt Text} & \rot{Cross Platform} & \rot{Availability} & \rot{Objectivity} & \rot{Hate words} & \rot{Spelling and Grammar} & \rot{Content Variety} & \rot{Date related} &  \rot{End with new line} & \rot{Emoji Lint}\\
%  & \rot{Checkable} & \rot{Customizable} & \rot{Blamable} & \rot{Fixable} & \rot{Execution} & \rot{Code snippets formatting} & \rot{Link Foramtting} & \rot{Link validation} & \rot{Formatting/Styling} & \rot{Style consistency} & \rot{Structure} & \rot{Terminology} & \rot{Sesitive content} & \rot{Best practices} & \rot{Timeliness} & \rot{Sections Completeness} & \rot{Repetition} & \rot{Sentence Length} & \rot{Too concise} & \rot{TOC} & \rot{Navigation} & \rot{No jargon} & \rot{Internal Links} & \rot{Visual Clarity} & \rot{Alt Text} & \rot{Cross Platform} & \rot{Availability} & \rot{Objectivity} & \rot{Ambiguity Understandability} & \rot{Quick Start} & \rot{Hate words} & \rot{Content Check/Tone} & \rot{Value-added} & \rot{Spelling} & \rot{Grammar} & \rot{Content Variety} & \rot{Demo link} & \rot{Date related} & \rot{End with new line} & \rot{Emoji Lint}\\
% Name & 
% \multicolumn{4}{c|}{Ladder} &
% % &
% % &
% % &
% \multicolumn{4}{c|}{Acc./Reliability} &
% % &
% % &
% % &
% \multicolumn{4}{c|}{ Consistency} &
% % &
% % &
% % &
% \multicolumn{2}{c|}{Security} &
% % &
% \multicolumn{2}{c|}{ Timeliness} &
% % &
% \multicolumn{3}{c|}{ Concise} &
% % &
% % &
% \multicolumn{7}{c|}{ Accessibility} &
% % &
% % &
% % &
% % &
% % &
% % &
% \multicolumn{1}{c|}{ } &
% \multicolumn{2}{c|}{ Objectivity} &
% % &
% \multicolumn{1}{c|}{ } &
% \multicolumn{2}{c|}{ Reputation} &
% % &
% \multicolumn{1}{c|}{ Value-added} &
% \multicolumn{2}{c|}{ Quality} &
% % &
% \multicolumn{2}{c|}{ Appeal} &
% % &
% \multicolumn{2}{c|}{ Others} &
% % &
% \\
% \midrule  

% alex~\cite{alex}\hspace{1mm} & \yes & \yes & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no\\
% awesome-lint~\cite{awesome_lint}\hspace{1mm} & \yes & \maybe & \yes & \yes & \no & \yes & \yes & \yes & \yes & \yes & \maybe & \maybe & \no & \no & \no & \maybe & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \maybe & \no & \no & \no & \yes & \no\\
% content-linter~\cite{github_content_linter}\hspace{1mm} & \yes & \maybe & \yes & \yes & \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \maybe & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \no & \maybe & \yes & \no\\
% % joblint & \yes & \yes & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no\\
% % MarkdownEditing & \yes & \yes & \no data available & \no data available & \no & \yes & \yes & \no & \yes & \yes & \no & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no\\
% markdownlint~\cite{markdownlint_ruby}\hspace{1mm} & \yes & \yes & \yes & \no & \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no\\
% DavidAnson markdownlint~\cite{markdownlint_node}\hspace{1mm} & \yes & \yes & \yes & \yes & \no & \yes & \yes & \no & \yes & \yes & \maybe & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \maybe & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \yes & \no\\
% mdformat~\cite{mdformat}\hspace{1mm} & \yes & \maybe & \no & \yes & \no & \yes & \yes & \no & \maybe & \yes & \maybe & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no\\
% mdsf & \maybe & \maybe & \maybe & \maybe & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no\\
% mdspell & \yes & \yes & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no\\
% proselint~\cite{proselint}\hspace{1mm} & \yes & \yes & \yes & \yes & \no & \no & \yes & \yes & \no & \maybe & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \yes & \no & \no & \yes & \no & \no & \yes & \yes & \no & \no & \maybe & \no & \no\\
% remark-lint~\cite{remarklint}\hspace{1mm} & \yes & \yes & \yes & \yes & \no & \yes & \yes & \yes & \yes & \yes & \maybe & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \maybe & \no & \no & \no & \yes & \yes\\
% standard-readme~\cite{standardreadme}\hspace{1mm} & \yes & \no  & \yes & \yes & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no\\
% textlint~\cite{textlint}\hspace{1mm} & \yes & \yes & \yes & \yes & \no & \no & \yes & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \maybe & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \yes & \yes & \no & \no & \maybe & \no & \no\\
% vale~\cite{vale}\hspace{1mm} & \yes & \yes & \yes & \yes & \no & \yes & \no & \no & \no & \maybe & \no & \maybe & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \yes & \no & \no & \no & \no & \no\\
% webhint~\cite{webhintio_org}\hspace{1mm} & \yes & \yes & \yes & \yes & \no & \no & \yes & \yes & \maybe & \maybe & \no & \no & \yes & \no & \no & \no & \no & \yes & \no & \no & \maybe & \no & \no & \yes & \yes & \yes & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no\\
% write-good~\cite{writegood}\hspace{1mm} & \yes & \yes & \yes & \maybe & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \no & \no & \no & \no & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \no\\
% grammarly~\cite{grammarly_website}\hspace{1mm} & \yes & \maybe & \yes & \yes & \no & \no & \maybe & \no & \no & \no & \no & \maybe & \no & \no & \no & \no & \maybe & \yes & \maybe & \no & \no & \yes & \no & \no & \no & \no & \no & \no & \yes & \no & \yes & \yes & \no & \yes & \yes & \no & \no & \yes & \no & \no\\

% \hline
% \textbf{\emph{LintMe}} &  \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes & \yes \\
%  \bottomrule
%         \end{tabular}}\\
%         \textbf{Y} = Supported, \textbf{N} = Not Supported, \textbf{P} = Partially Supported.

% \end{table*}

==> figures/recipe-rules.tex <==
\begin{table}[t]
\centering
\caption{The set of rules used to lint recipes. These are grouped together in playground preset called ``Recipe Rules''.}
\label{tab:recipe-rules}
% \footnotesize{}
\small
\begin{tabular}{|p{4.5cm}|p{9.5cm}|}
\hline
\textbf{Rule} & \textbf{Description}  \\
\hline
\lint{metric-and-imperial-weight-units} &
Require weights to be given in both metric (g, kg) and US imperial (oz, lb) units.
\\
\hline
\lint{generic-ingredient-names} &
Use generic ingredient names instead of brand names.
\\
\hline
\lint{ingredients-ordering} &
Ensure ingredients are listed in the order of their first use in the instructions.
\\
\hline
\lint{nested-list-items} &
Fail if any instruction step asks the cook to do two tasks at once.
\\
\hline
\lint{require-buy-and-use-amounts} &
Require each recipe to specify both the quantity to buy and the amount to use.
\\
\hline
\lint{require-prep-or-total-time} &
Require the recipe to include either a prep time or a total time.
\\
\hline
\lint{section-completeness} &
Ensure the recipe includes both an Ingredients section and a Preparation section.
\\
\hline
\lint{substitutions-section-check} &
Check for a Substitutions section and suggest moving it to the end if not last.
\\
\hline
\lint{temperature-format-check} &
Ensure temperatures include a space before a capital “F”.
\\
\hline
\lint{temperature-missing-unit} &
Flag temperatures written with a degree symbol but missing a unit.
\\
\hline
\lint{unknown-timer-units} &
Fail if time durations use abbreviations; require full words (seconds, minutes, hours).
\\
\hline
\lint{weight-and-volume} &
Require each ingredient to list a weight, volume, or count.
\\
\hline
\end{tabular}
\end{table}

